KD-Club: An Efficient Exact Algorithm with New Coloring-based Upper Bound for the Maximum k-Defective Clique Problem

The Maximum k-Defective Clique Problem (MDCP) aims to find a maximum k-defective clique in a given graph, where a k-defective clique is a relaxation clique missing at most k edges. MDCP is NP-hard and finds many real-world applications in analyzing dense but not necessarily complete subgraphs. Exact algorithms for MDCP mainly follow the Branch-and-bound (BnB) framework, whose performance heavily depends on the quality of the upper bound on the cardinality of a maximum k-defective clique. The state-of-the-art BnB MDCP algorithms calculate the upper bound quickly but conservatively as they ignore many possible missing edges. In this paper, we propose a novel CoLoring-based Upper Bound (CLUB) that uses graph coloring techniques to detect independent sets so as to detect missing edges ignored by the previous methods. We then develop a new BnB algorithm for MDCP, called KD-Club, using CLUB in both the preprocessing stage for graph reduction and the BnB searching process for branch pruning. Extensive experiments show that KD-Club significantly outperforms state-of-the-art BnB MDCP algorithms on the number of solved instances within the cut-off time, having much smaller search tree and shorter solving time on various benchmarks.

==> tabs/comp-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\centering
\footnotesize
%\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc}\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{~~$k$}} & \multicolumn{3}{c|}{Facebook} & \multicolumn{3}{c|}{Realworld} & \multicolumn{3}{c|}{SNAP and DIMACS10} & \multicolumn{3}{c}{DIMACS2} \\
\multicolumn{1}{c|}{}                   & KD-Club     & KDBB    & MADEC$^+$    & KD-Club     & KDBB     & MADEC$^+$    & KD-Club        & KDBB       & MADEC$^+$       & KD-Club    & KDBB    & MADEC$^+$   \\ \hline
~~1                                       & \textbf{112}      & 110     & 12      & \textbf{130}      & 124      & 81      & \textbf{39}          & \textbf{39}         & 24          & 31      & 17      & \textbf{32}      \\
~~3                                       & \textbf{112}      & 110     & ~~0      & \textbf{125}      & 116      & 62      & \textbf{38}          & \textbf{38}         & 23          & \textbf{27}      & 12      & 14      \\
~~5                                       & \textbf{111}      & 109     & ~~0      & \textbf{121}      & 110      & 52       & 37          & \textbf{38}         & 23          & \textbf{25}      & 12      & 12      \\
10                                      & \textbf{109}      & 108     & ~~0       & \textbf{106}      & ~~94       & 28       & \textbf{34}          & \textbf{34}         & 11          & \textbf{19}      & 11      & ~~6       \\
15                                      & \textbf{108}      & 104     & ~~0        & ~~\textbf{94}       & ~~70       & 22       & \textbf{30}          & 28         & ~~9          & \textbf{13}      & 11      & ~~2       \\
20                                      & \textbf{104}      & ~~86      & ~~0        & ~~\textbf{85}       & ~~59       & 16       & \textbf{27}          & 24         & ~~6           & \textbf{12}      & 11      & ~~1      
\\\bottomrule
\end{tabular}
%}

\caption{Summarized results of KD-Club, KDBB, and MADEC$^+$ on four benchmarks. The best results appear in bold.}
\label{tab-comp-results}
\end{table*}

%

==> tabs/detailed_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
%\fontsize{9pt}{15}
\footnotesize
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lrr|rrrr:rrrr|rrrr:rrrr}\toprule
\multicolumn{1}{l}{\multirow{3}{*}{Instance}} & \multicolumn{1}{r}{\multirow{3}{*}{$|V|$}} & \multicolumn{1}{r|}{\multirow{3}{*}{$|E|$}} & \multicolumn{8}{c|}{$k=3$}                                                                                                                                                                                           & \multicolumn{8}{c}{$k=10$}                                                                                                                                                                                          \\ \cline{4-19} 
\multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                     & \multicolumn{1}{c|}{}                     & \multicolumn{4}{c:}{KD-Club}                                                                                & \multicolumn{4}{c|}{KDBB}                                                                                & \multicolumn{4}{c:}{KD-Club}                                                                                & \multicolumn{4}{c}{KDBB}                                                                                \\
\multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                     & \multicolumn{1}{c|}{}                     & \multicolumn{1}{r}{$|V'|$} & \multicolumn{1}{r}{$|E'|$} & \multicolumn{1}{r}{Tree} & \multicolumn{1}{r:}{Time} & \multicolumn{1}{r}{$|V'|$} & \multicolumn{1}{r}{$|E'|$} & \multicolumn{1}{r}{Tree} & \multicolumn{1}{r|}{Time} & \multicolumn{1}{r}{$|V'|$} & \multicolumn{1}{r}{$|E'|$} & \multicolumn{1}{r}{Tree} & \multicolumn{1}{r:}{Time} & \multicolumn{1}{r}{$|V'|$} & \multicolumn{1}{r}{$|E'|$} & \multicolumn{1}{r}{Tree} & \multicolumn{1}{r}{Time} \\ \hline
C125-9                                         & 125                                      & 6963                                      & 125                     & 6963                    & \textbf{35.83}           & \textbf{23.83}           & 125                     & 6963                    & NA                       & NA                        & 125                     & 6963                    & \textbf{535.6}           & \textbf{137.2}           & 125                     & 6963                    & NA                       & NA                       \\
gen200-p0-9-55                                 & 200                                      & 17910                                     & 200                     & 17910                   & \textbf{45.68}           & \textbf{102.4}           & 200                     & 17910                   & NA                       & NA                        & 200                     & 17910                   & \textbf{324.6}           & \textbf{275.1}           & 200                     & 17910                   & NA                       & NA                       \\
ia-wiki-Talk                                   & 92117                                    & 360767                                    & 179                     & 2244                    & \textbf{0.042}           & \textbf{2.947}           & 1119                    & 46194                   & NA                       & NA                        & 2492                    & 68463                   & \textbf{334.0}           & \textbf{1420}            & 9424                    & 155317                  & NA                       & NA                       \\
johnson8-4-4                                   & 70                                       & 1855                                      & 70                      & 1855                    & \textbf{3.717}           & \textbf{0.961}           & 70                      & 1855                    & 184.2                    & 33.62                     & 70                      & 1855                    & \textbf{3436}            & \textbf{338.5}           & 70                      & 1855                    & NA                       & NA                       \\
MANN-a27                                       & 378                                      & 70551                                     & 378                     & 70551                   & \textbf{101.9}           & \textbf{460.1}           & 378                     & 70551                   & NA                       & NA                        & 378                     & 70551                   & \textbf{99.94}           & \textbf{468.7}           & 378                     & 70551                   & NA                       & NA                       \\
san200-0-7-1                                   & 200                                      & 13930                                     & 200                     & 13930                   & \textbf{0.866}           & \textbf{2.789}           & 200                     & 13930                   & NA                       & NA                        & 200                     & 13930                   & \textbf{36.93}           & \textbf{34.16}           & 200                     & 13930                   & NA                       & NA                       \\
scc\_rt\_lebanon                               & 3370                                     & 5                                         & 3370                    & 5                       & \textbf{0.002}           & \textbf{1.170}           & 3370                    & 5                       & 1135                     & 169.4                     & 3370                    & 5                       & \textbf{0.005}           & \textbf{1.183}           & 3370                    & 5                       & NA                       & NA                       \\
Slashdot0811                                   & 77360                                    & 469180                                    & 138                     & 5411                    & \textbf{0.140}           & \textbf{0.653}           & 246                     & 9888                    & 65.67                    & 80.92                     & 210                     & 7787                    & \textbf{15.31}           & \textbf{10.03}           & 503                     & 16319                   & 428.3                    & 75.79                    \\
soc-digg                                       & 770799                                   & 5907132                                   & 199                     & 13551                   & \textbf{0.607}           & \textbf{69.97}           & 5580                    & 875610                  & NA                       & NA                        & 519                     & 37458                   & \textbf{29.27}           & \textbf{214.0}           & 7349                    & 1141673                 & NA                       & NA                       \\
socfb-Auburn71                                 & 18448                                    & 973918                                    & 116                     & 5780                    & \textbf{0.060}           & \textbf{8.102}           & 1048                    & 46693                   & 23.01                    & 27.51                     & 323                     & 14989                   & \textbf{5.589}           & \textbf{22.70}           & 1624                    & 73790                   & 138.0                    & 73.20                    \\
%socfb-Berkeley13                               & 22900                                    & 852419                                    & 128                     & 3776                    & \textbf{0.045}           & \textbf{3.776}           & 925                     & 29206                   & 2.212                    & 6.487                     & 591                     & 17281                   & \textbf{1.099}           & \textbf{15.50}           & 10                      & 1817                    & 10.94                    & 35.16                    \\
socfb-Cornell5                                 & 18660                                    & 790777                                    & 211                     & 6552                    & \textbf{0.056}           & \textbf{4.450}           & 1292                    & 52540                   & 22.57                    & 89.23                     & 541                     & 15848                   & \textbf{0.825}           & \textbf{22.60}           & 2174                    & 84381                   & 44.67                    & 107.1                    \\
socfb-Duke14                                   & 9885                                     & 506437                                    & 198                     & 4714                    & \textbf{0.054}           & \textbf{10.32}           & 1489                    & 56078                   & 155.1                    & 601.1                     & 1042                    & 34631                   & \textbf{39.14}           & \textbf{127.1}           & 3375                    & 134029                  & 1416                     & 1863                     \\
socfb-FSU53                                    & 27737                                    & 1034802                                   & 188                     & 8235                    & \textbf{0.052}           & \textbf{8.259}           & 642                     & 29659                   & 39.75                    & 34.89                     & 401                     & 18587                   & \textbf{1.161}           & \textbf{12.57}           & 1025                    & 45290                   & 173.2                    & 53.67                    \\
socfb-Indiana                                  & 29732                                    & 1305757                                   & 136                     & 4394                    & \textbf{0.036}           & \textbf{7.915}           & 1596                    & 57741                   & 2.839                    & 22.20                     & 844                     & 29290                   & \textbf{1.065}           & \textbf{17.54}           & 2884                    & 104681                  & 16.84                    & 151.5                    \\
socfb-Michigan23                               & 30147                                    & 1176516                                   & 218                     & 5764                    & \textbf{0.048}           & \textbf{5.805}           & 1133                    & 42875                   & 2.090                    & 13.34                     & 542                     & 18091                   & \textbf{0.658}           & \textbf{12.30}           & 2378                    & 95042                   & 10.72                    & 118.4                    \\
socfb-MIT                                      & 6402                                     & 251230                                    & 203                     & 4806                    & \textbf{0.044}           & \textbf{5.435}           & 1099                    & 35822                   & 3.866                    & 10.29                     & 977                     & 28110                   & \textbf{3.196}           & \textbf{35.87}           & 1949                    & 74120                   & 36.62                    & 76.38                    \\
socfb-Oklahoma97                               & 17425                                    & 892528                                    & 79                      & 2958                    & \textbf{0.049}           & \textbf{11.46}           & 1148                    & 61418                   & 166.7                    & 203.2                     & 362                     & 18706                   & \textbf{6.396}           & \textbf{16.35}           & 1733                    & 90058                   & 615.2                    & 234.1                    \\
socfb-OR                                       & 63392                                    & 816886                                    & 152                     & 2901                    & \textbf{0.075}           & \textbf{2.091}           & 1440                    & 35123                   & 5.209                    & 11.97                     & 621                     & 14999                   & \textbf{2.650}           & \textbf{23.49}           & 4910                    & 117554                  & 42.24                    & 510.8                    \\
socfb-Penn94                                   & 41536                                    & 1362220                                   & 71                      & 2228                    & \textbf{0.043}           & \textbf{4.693}           & 875                     & 23454                   & 1.065                    & 4.855                     & 237                     & 6564                    & \textbf{0.420}           & \textbf{7.032}           & 2087                    & 58201                   & 2.863                    & 34.31                    \\
socfb-Rice31                                   & 4087                                     & 184828                                    & 83                      & 1601                    & \textbf{0.033}           & \textbf{2.363}           & 1170                    & 36409                   & 10.86                    & 16.85                     & 921                     & 25731                   & \textbf{2.337}           & \textbf{35.17}           & 2161                    & 87191                   & 80.34                    & 141.8                    \\
socfb-Tennessee95                              & 16979                                    & 770659                                    & 87                      & 3604                    & \textbf{0.055}           & \textbf{4.836}           & 802                     & 31594                   & 32.99                    & 19.18                     & 199                     & 8737                    & \textbf{0.635}           & \textbf{10.03}           & 1352                    & 55156                   & 72.43                    & 36.94                    \\
socfb-Texas84                                  & 36364                                    & 1590651                                   & 129                     & 6606                    & \textbf{0.147}           & \textbf{8.989}           & 927                     & 41536                   & 85.40                    & 101.0                     & 461                     & 18985                   & \textbf{17.57}           & \textbf{40.66}           & 1494                    & 66131                   & 600.9                    & 398.6                    \\
socfb-UF                                       & 35111                                    & 1465654                                   & 299                     & 10983                   & \textbf{0.064}           & \textbf{15.21}           & 1612                    & 75851                   & 54.72                    & 82.69                     & 975                     & 42128                   & \textbf{5.514}           & \textbf{110.8}           & 2088                    & 98361                   & 236.7                    & 159.3                    \\
socfb-UGA50                                    & 24389                                    & 1174057                                   & 125                     & 6457                    & \textbf{0.099}           & \textbf{7.867}           & 1276                    & 55310                   & 80.32                    & 103.2                     & 457                     & 18956                   & \textbf{11.41}           & \textbf{39.75}           & 2093                    & 89760                   & 471.5                    & 286.4                    \\
socfb-Uillinois                                & 30795                                    & 1264421                                   & 104                     & 4828                    & \textbf{0.062}           & \textbf{6.582}           & 586                     & 25096                   & 13.98                    & 13.07                     & 232                     & 11219                   & \textbf{1.196}           & \textbf{8.368}           & 1028                    & 43222                   & 76.21                    & 27.78                    \\
socfb-UMass92                                  & 16516                                    & 519385                                    & 142                     & 3251                    & \textbf{0.034}           & 1.636                    & 634                     & 14250                   & 0.848                    & \textbf{1.489}            & 523                     & 12242                   & \textbf{0.819}           & \textbf{3.267}           & 1440                    & 37824                   & 4.214                    & 13.40                    \\
socfb-UVA16                                    & 17196                                    & 789321                                    & 213                     & 6905                    & \textbf{0.065}           & 4.486                    & 723                     & 24976                   & 2.724                    & \textbf{4.334}            & 639                     & 19899                   & \textbf{4.048}           & \textbf{22.61}           & 1818                    & 66673                   & 38.56                    & 55.52                    \\
socfb-Vassar85                                 & 3068                                     & 119161                                    & 80                      & 1220                    & \textbf{0.018}           & \textbf{0.654}           & 940                     & 22547                   & 0.545                    & 3.356                     & 496                     & 9340                    & \textbf{1.398}           & \textbf{18.27}           & 2591                    & 99363                   & 7.661                    & 220.9                    \\
socfb-Wisconsin87                              & 23831                                    & 835946                                    & 122                     & 3340                    & \textbf{0.037}           & \textbf{3.418}           & 974                     & 30242                   & 4.655                    & 8.164                     & 727                     & 20457                   & \textbf{2.280}           & \textbf{17.83}           & 2371                    & 72240                   & 38.35                    & 81.10                    \\
socfb-wosn-friends                             & 63731                                    & 817090                                    & 152                     & 2901                    & \textbf{0.075}           & \textbf{2.109}           & 1440                    & 35123                   & 5.209                    & 12.13                     & 621                     & 14999                   & \textbf{2.650}           & \textbf{24.45}           & 4910                    & 117554                  & 42.24                    & 514.0                    \\
socfb-Yale4                                    & 8578                                     & 405450                                    & 140                     & 3145                    & \textbf{0.026}           & \textbf{2.622}           & 1033                    & 28691                   & 4.345                    & 7.870                     & 809                     & 20248                   & \textbf{1.192}           & \textbf{31.41}           & 2883                    & 95160                   & 31.38                    & 160.6                    \\
Wiki-Vote                                      & 7115                                     & 100762                                    & 85                      & 1602                    & \textbf{0.104}           & \textbf{1.392}           & 902                     & 34228                   & 182.2                    & 430.5                     & 1378                    & 40535                   & \textbf{40.36}           & \textbf{170.8}           & 2233                    & 72679                   & NA                       & NA            \\ \bottomrule          
\end{tabular}
}
\caption{Detailed results of KD-Club and KDBB on 32 representative MDCP instances from four benchmarks with $k = 3$ and $k=10$. The search tree size is in $10^4$, and the time is in seconds. The better results appear in bold.}
\label{tab-detailed-result}
\end{table*}

==> tabs/detailed_results2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
%\fontsize{9pt}{15}
\footnotesize
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{lrr|rrrr:rrrr|rrrr:rrrr}\toprule
\multicolumn{1}{l}{\multirow{3}{*}{Instance}} & \multicolumn{1}{r}{\multirow{3}{*}{\hspace{-0.75em}$|V|$}} & \multicolumn{1}{r|}{\multirow{3}{*}{\hspace{-0.75em}$|E|$}} & \multicolumn{8}{c|}{$k=3$}                                                                                                                                                                                           & \multicolumn{8}{c}{$k=10$}                                                                                                                                                                                          \\ \cline{4-19} 
\multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                     & \multicolumn{1}{c|}{}                     & \multicolumn{4}{c:}{KD-Club}                                                                                & \multicolumn{4}{c|}{KDBB}                                                                                & \multicolumn{4}{c:}{KD-Club}                                                                                & \multicolumn{4}{c}{KDBB}                                                                                \\
\multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                     & \multicolumn{1}{c|}{}                     & \multicolumn{1}{r}{$|V'|$} & \multicolumn{1}{r}{$|E'|$} & \multicolumn{1}{r}{Tree} & \multicolumn{1}{r:}{Time} & \multicolumn{1}{r}{$|V'|$} & \multicolumn{1}{r}{$|E'|$} & \multicolumn{1}{r}{Tree} & \multicolumn{1}{r|}{Time} & \multicolumn{1}{r}{$|V'|$} & \multicolumn{1}{r}{$|E'|$} & \multicolumn{1}{r}{Tree} & \multicolumn{1}{r:}{Time} & \multicolumn{1}{r}{$|V'|$} & \multicolumn{1}{r}{$|E'|$} & \multicolumn{1}{r}{Tree} & \multicolumn{1}{r}{Time} \\ \hline
C125-9                                         & \hspace{-0.75em}125                                      & \hspace{-0.75em}6963                                      & 125                     & 6963                    & \textbf{35.83}           & \textbf{23.83}           & 125                     & 6963                    & NA                       & NA                        & 125                     & 6963                    & \textbf{535.6}           & \textbf{137.2}           & 125                     & 6963                    & NA                       & NA                       \\
gen200-p0-9-55                                 & 200                                      & 17910                                     & 200                     & 17910                   & \textbf{45.68}           & \textbf{102.4}           & \hspace{-0.75em}200                     & \hspace{-0.75em}17910                   & NA                       & NA                        & 200                     & 17910                   & \textbf{324.6}           & \textbf{275.1}           & 200                     & 17910                   & NA                       & NA                       \\
ia-wiki-Talk                                   & \hspace{-0.75em}92117                                    & \hspace{-0.75em}360767                                    & 179                     & 2244                    & \textbf{0.042}           & \textbf{2.947}           & 1119                    & 46194                   & NA                       & NA                        & 2492                    & 68463                   & \textbf{334.0}           & \textbf{1420}            & 9424                    & 155317                  & NA                       & NA                       \\
johnson8-4-4                                   & \hspace{-0.75em}70                                       & \hspace{-0.75em}1855                                      & 70                      & 1855                    & \textbf{3.717}           & \textbf{0.961}           & 70                      & 1855                    & 184.2                    & 33.62                     & 70                      & 1855                    & \textbf{3436}            & \textbf{338.5}           & 70                      & 1855                    & NA                       & NA                       \\
MANN-a27                                       & \hspace{-0.75em}378                                      & \hspace{-0.75em}70551                                     & 378                     & 70551                   & \textbf{101.9}           & \textbf{460.1}           & 378                     & 70551                   & NA                       & NA                        & 378                     & 70551                   & \textbf{99.94}           & \textbf{468.7}           & 378                     & 70551                   & NA                       & NA                       \\
san200-0-7-1                                   & \hspace{-0.75em}200                                      & \hspace{-0.75em}13930                                     & 200                     & 13930                   & \textbf{0.866}           & \textbf{2.789}           & 200                     & 13930                   & NA                       & NA                        & 200                     & 13930                   & \textbf{36.93}           & \textbf{34.16}           & 200                     & 13930                   & NA                       & NA                       \\
scc\_rt\_lebanon                               & \hspace{-0.75em}3370                                     & \hspace{-0.75em}5                                         & 3370                    & 5                       & \textbf{0.002}           & \textbf{1.170}           & 3370                    & 5                       & 1135                     & 169.4                     & 3370                    & 5                       & \textbf{0.005}           & \textbf{1.183}           & 3370                    & 5                       & NA                       & NA                       \\
Slashdot0811                                   & \hspace{-0.75em}77360                                    & \hspace{-0.75em}469180                                    & 138                     & 5411                    & \textbf{0.140}           & \textbf{0.653}           & 246                     & 9888                    & 65.67                    & 80.92                     & 210                     & 7787                    & \textbf{15.31}           & \textbf{10.03}           & 503                     & 16319                   & 428.3                    & 75.79                    \\
soc-digg                                       & \hspace{-0.75em}770799                                   & \hspace{-0.75em}5907132                                   & 199                     & 13551                   & \textbf{0.607}           & \textbf{69.97}           & 5580                    & 875610                  & NA                       & NA                        & 519                     & 37458                   & \textbf{29.27}           & \textbf{214.0}           & 7349                    & 1141673                 & NA                       & NA                       \\
socfb-Auburn71                                 & \hspace{-0.75em}18448                                    & \hspace{-0.75em}973918                                    & 116                     & 5780                    & \textbf{0.060}           & \textbf{8.102}           & 1048                    & 46693                   & 23.01                    & 27.51                     & 323                     & 14989                   & \textbf{5.589}           & \textbf{22.70}           & 1624                    & 73790                   & 138.0                    & 73.20                    \\
%socfb-Berkeley13                               & 22900                                    & 852419                                    & 128                     & 3776                    & \textbf{0.045}           & \textbf{3.776}           & 925                     & 29206                   & 2.212                    & 6.487                     & 591                     & 17281                   & \textbf{1.099}           & \textbf{15.50}           & 10                      & 1817                    & 10.94                    & 35.16                    \\
socfb-Cornell5                                 & \hspace{-0.75em}18660                                    & \hspace{-0.75em}790777                                    & 211                     & 6552                    & \textbf{0.056}           & \textbf{4.450}           & 1292                    & 52540                   & 22.57                    & 89.23                     & 541                     & 15848                   & \textbf{0.825}           & \textbf{22.60}           & 2174                    & 84381                   & 44.67                    & 107.1                    \\
socfb-Duke14                                   & \hspace{-0.75em}9885                                     & \hspace{-0.75em}506437                                    & 198                     & 4714                    & \textbf{0.054}           & \textbf{10.32}           & 1489                    & 56078                   & 155.1                    & 601.1                     & 1042                    & 34631                   & \textbf{39.14}           & \textbf{127.1}           & 3375                    & 134029                  & 1416                     & 1863                     \\
socfb-FSU53                                    & \hspace{-0.75em}27737                                    & \hspace{-0.75em}1034802                                   & 188                     & 8235                    & \textbf{0.052}           & \textbf{8.259}           & 642                     & 29659                   & 39.75                    & 34.89                     & 401                     & 18587                   & \textbf{1.161}           & \textbf{12.57}           & 1025                    & 45290                   & 173.2                    & 53.67                    \\
socfb-Indiana                                  & \hspace{-0.75em}29732                                    & \hspace{-0.75em}1305757                                   & 136                     & 4394                    & \textbf{0.036}           & \textbf{7.915}           & 1596                    & 57741                   & 2.839                    & 22.20                     & 844                     & 29290                   & \textbf{1.065}           & \textbf{17.54}           & 2884                    & 104681                  & 16.84                    & 151.5                    \\
socfb-Michigan23                               & \hspace{-0.75em}30147                                    & \hspace{-0.75em}1176516                                   & 218                     & 5764                    & \textbf{0.048}           & \textbf{5.805}           & 1133                    & 42875                   & 2.090                    & 13.34                     & 542                     & 18091                   & \textbf{0.658}           & \textbf{12.30}           & 2378                    & 95042                   & 10.72                    & 118.4                    \\
socfb-MIT                                      & \hspace{-0.75em}6402                                     & \hspace{-0.75em}251230                                    & 203                     & 4806                    & \textbf{0.044}           & \textbf{5.435}           & 1099                    & 35822                   & 3.866                    & 10.29                     & 977                     & 28110                   & \textbf{3.196}           & \textbf{35.87}           & 1949                    & 74120                   & 36.62                    & 76.38                    \\
socfb-Oklahoma97                               & \hspace{-0.75em}17425                                    & \hspace{-0.75em}892528                                    & 79                      & 2958                    & \textbf{0.049}           & \textbf{11.46}           & 1148                    & 61418                   & 166.7                    & 203.2                     & 362                     & 18706                   & \textbf{6.396}           & \textbf{16.35}           & 1733                    & 90058                   & 615.2                    & 234.1                    \\
socfb-OR                                       & \hspace{-0.75em}63392                                    & \hspace{-0.75em}816886                                    & 152                     & 2901                    & \textbf{0.075}           & \textbf{2.091}           & 1440                    & 35123                   & 5.209                    & 11.97                     & 621                     & 14999                   & \textbf{2.650}           & \textbf{23.49}           & 4910                    & 117554                  & 42.24                    & 510.8                    \\
socfb-Penn94                                   & \hspace{-0.75em}41536                                    & \hspace{-0.75em}1362220                                   & 71                      & 2228                    & \textbf{0.043}           & \textbf{4.693}           & 875                     & 23454                   & 1.065                    & 4.855                     & 237                     & 6564                    & \textbf{0.420}           & \textbf{7.032}           & 2087                    & 58201                   & 2.863                    & 34.31                    \\
socfb-Rice31                                   & \hspace{-0.75em}4087                                     & \hspace{-0.75em}184828                                    & 83                      & 1601                    & \textbf{0.033}           & \textbf{2.363}           & 1170                    & 36409                   & 10.86                    & 16.85                     & 921                     & 25731                   & \textbf{2.337}           & \textbf{35.17}           & 2161                    & 87191                   & 80.34                    & 141.8                    \\
socfb-Tennessee95                              & \hspace{-0.75em}16979                                    & \hspace{-0.75em}770659                                    & 87                      & 3604                    & \textbf{0.055}           & \textbf{4.836}           & 802                     & 31594                   & 32.99                    & 19.18                     & 199                     & 8737                    & \textbf{0.635}           & \textbf{10.03}           & 1352                    & 55156                   & 72.43                    & 36.94                    \\
socfb-Texas84                                  & \hspace{-0.75em}36364                                    & \hspace{-0.75em}1590651                                   & 129                     & 6606                    & \textbf{0.147}           & \textbf{8.989}           & 927                     & 41536                   & 85.40                    & 101.0                     & 461                     & 18985                   & \textbf{17.57}           & \textbf{40.66}           & 1494                    & 66131                   & 600.9                    & 398.6                    \\
socfb-UF                                       & \hspace{-0.75em}35111                                    & \hspace{-0.75em}1465654                                   & 299                     & 10983                   & \textbf{0.064}           & \textbf{15.21}           & 1612                    & 75851                   & 54.72                    & 82.69                     & 975                     & 42128                   & \textbf{5.514}           & \textbf{110.8}           & 2088                    & 98361                   & 236.7                    & 159.3                    \\
socfb-UGA50                                    & \hspace{-0.75em}24389                                    & \hspace{-0.75em}1174057                                   & 125                     & 6457                    & \textbf{0.099}           & \textbf{7.867}           & 1276                    & 55310                   & 80.32                    & 103.2                     & 457                     & 18956                   & \textbf{11.41}           & \textbf{39.75}           & 2093                    & 89760                   & 471.5                    & 286.4                    \\
socfb-Uillinois                                & \hspace{-0.75em}30795                                    & \hspace{-0.75em}1264421                                   & 104                     & 4828                    & \textbf{0.062}           & \textbf{6.582}           & 586                     & 25096                   & 13.98                    & 13.07                     & 232                     & 11219                   & \textbf{1.196}           & \textbf{8.368}           & 1028                    & 43222                   & 76.21                    & 27.78                    \\
socfb-UMass92                                  & \hspace{-0.75em}16516                                    & \hspace{-0.75em}519385                                    & 142                     & 3251                    & \textbf{0.034}           & 1.636                    & 634                     & 14250                   & 0.848                    & \textbf{1.489}            & 523                     & 12242                   & \textbf{0.819}           & \textbf{3.267}           & 1440                    & 37824                   & 4.214                    & 13.40                    \\
socfb-UVA16                                    & \hspace{-0.75em}17196                                    & \hspace{-0.75em}789321                                    & 213                     & 6905                    & \textbf{0.065}           & 4.486                    & 723                     & 24976                   & 2.724                    & \textbf{4.334}            & 639                     & 19899                   & \textbf{4.048}           & \textbf{22.61}           & 1818                    & 66673                   & 38.56                    & 55.52                    \\
socfb-Vassar85                                 & \hspace{-0.75em}3068                                     & \hspace{-0.75em}119161                                    & 80                      & 1220                    & \textbf{0.018}           & \textbf{0.654}           & 940                     & 22547                   & 0.545                    & 3.356                     & 496                     & 9340                    & \textbf{1.398}           & \textbf{18.27}           & 2591                    & 99363                   & 7.661                    & 220.9                    \\
socfb-Wisconsin87                              & \hspace{-0.75em}23831                                    & \hspace{-0.75em}835946                                    & 122                     & 3340                    & \textbf{0.037}           & \textbf{3.418}           & 974                     & 30242                   & 4.655                    & 8.164                     & 727                     & 20457                   & \textbf{2.280}           & \textbf{17.83}           & 2371                    & 72240                   & 38.35                    & 81.10                    \\
socfb-wosn-friends                             & \hspace{-0.75em}63731                                    & \hspace{-0.75em}817090                                    & 152                     & 2901                    & \textbf{0.075}           & \textbf{2.109}           & 1440                    & 35123                   & 5.209                    & 12.13                     & 621                     & 14999                   & \textbf{2.650}           & \textbf{24.45}           & 4910                    & 117554                  & 42.24                    & 514.0                    \\
socfb-Yale4                                    & \hspace{-0.75em}8578                                     & \hspace{-0.75em}405450                                    & 140                     & 3145                    & \textbf{0.026}           & \textbf{2.622}           & 1033                    & 28691                   & 4.345                    & 7.870                     & 809                     & 20248                   & \textbf{1.192}           & \textbf{31.41}           & 2883                    & 95160                   & 31.38                    & 160.6                    \\
Wiki-Vote                                      & \hspace{-0.75em}7115                                     & \hspace{-0.75em}100762                                    & 85                      & 1602                    & \textbf{0.104}           & \textbf{1.392}           & 902                     & 34228                   & 182.2                    & 430.5                     & 1378                    & 40535                   & \textbf{40.36}           & \textbf{170.8}           & 2233                    & 72679                   & NA                       & NA            \\ \bottomrule          
\end{tabular}
% }
\caption{Detailed results of KD-Club and KDBB on 32 representative MDCP instances from four benchmarks with $k = 3$ and $k=10$. The search tree size is in $10^4$, and the time is in seconds. The better results appear in bold.}
\label{tab-detailed-result}
\end{table*}

==> tabs/detailed_results3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
%\fontsize{9pt}{15}
\footnotesize
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{lrr|rrrr:rrrr|rrrr:rrrr}\toprule
\multicolumn{1}{l}{\multirow{3}{*}{Instance}} & \multicolumn{1}{r}{\multirow{3}{*}{<>$|V|$}} & \multicolumn{1}{r|}{\multirow{3}{*}{<>$|E|$}} & \multicolumn{8}{c|}{$k=3$}                                                                                                                                                                                           & \multicolumn{8}{c}{$k=10$}                                                                                                                                                                                          \\ \cline{4-19} 
\multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                     & \multicolumn{1}{c|}{}                     & \multicolumn{4}{c:}{KD-Club}                                                                                & \multicolumn{4}{c|}{KDBB}                                                                                & \multicolumn{4}{c:}{KD-Club}                                                                                & \multicolumn{4}{c}{KDBB}                                                                                \\
\multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                     & \multicolumn{1}{c|}{}                     & \multicolumn{1}{r}{<>$|V'|$} & \multicolumn{1}{r}{<>$|E'|$} & \multicolumn{1}{r}{<>Tree} & \multicolumn{1}{r:}{<>Time} & \multicolumn{1}{r}{<>$|V'|$} & \multicolumn{1}{r}{<>$|E'|$} & \multicolumn{1}{r}{<>Tree} & \multicolumn{1}{r|}{<>Time} & \multicolumn{1}{r}{<>$|V'|$} & \multicolumn{1}{r}{<>$|E'|$} & \multicolumn{1}{r}{<>Tree} & \multicolumn{1}{r:}{<>Time} & \multicolumn{1}{r}{<>$|V'|$} & \multicolumn{1}{r}{<>$|E'|$} & \multicolumn{1}{r}{<>Tree} & \multicolumn{1}{r}{<>Time} \\ \hline
C125-9                                         & <>125                                      & <>6963                                      & <>125                     & <>6963                    & <>\textbf{35.83}           & <>\textbf{23.83}           & <>125                     & <>6963                    & <>NA                       & <>NA                        & <>125                     & <>6963                    & <>\textbf{535.6}           & <>\textbf{137.2}           & <>125                     & <>6963                    & <>NA                       & <>NA                       \\
gen200-p0-9-55                                 & <>200                                      & <>17910                                     & <>200                     & <>17910                   & <>\textbf{45.68}           & <>\textbf{102.4}           & <>200                     & <>17910                   & <>NA                       & <>NA                        & <>200                     & <>17910                   & <>\textbf{324.6}           & <>\textbf{275.1}           & <>200                     & <>17910                   & <>NA                       & <>NA                       \\
ia-wiki-Talk                                   & <>92117                                    & <>360767                                    & <>179                     & <>2244                    & <>\textbf{0.042}           & <>\textbf{2.947}           & <>1119                    & <>46194                   & <>NA                       & <>NA                        & <>2492                    & <>68463                   & <>\textbf{334.0}           & <>\textbf{1420}            & <>9424                    & <>155317                  & <>NA                       & <>NA                       \\
johnson8-4-4                                   & <>70                                       & <>1855                                      & <>70                      & <>1855                    & <>\textbf{3.717}           & <>\textbf{0.961}           & <>70                      & <>1855                    & <>184.2                    & <>33.62                     & <>70                      & <>1855                    & <>\textbf{3436}            & <>\textbf{338.5}           & <>70                      & <>1855                    & <>NA                       & <>NA                       \\
MANN-a27                                       & <>378                                      & <>70551                                     & <>378                     & <>70551                   & <>\textbf{101.9}           & <>\textbf{460.1}           & <>378                     & <>70551                   & <>NA                       & <>NA                        & <>378                     & <>70551                   & <>\textbf{99.94}           & <>\textbf{468.7}           & <>378                     & <>70551                   & <>NA                       & <>NA                       \\
san200-0-7-1                                   & <>200                                      & <>13930                                     & <>200                     & <>13930                   & <>\textbf{0.866}           & <>\textbf{2.789}           & <>200                     & <>13930                   & <>NA                       & <>NA                        & <>200                     & <>13930                   & <>\textbf{36.93}           & <>\textbf{34.16}           & <>200                     & <>13930                   & <>NA                       & <>NA                       \\
scc\_rt\_lebanon                               & <>3370                                     & <>5                                         & <>3370                    & <>5                       & <>\textbf{0.002}           & <>\textbf{1.170}           & <>3370                    & <>5                       & <>1135                     & <>169.4                     & <>3370                    & <>5                       & <>\textbf{0.005}           & <>\textbf{1.183}           & <>3370                    & <>5                       & <>NA                       & <>NA                       \\
Slashdot0811                                   & <>77360                                    & <>469180                                    & <>138                     & <>5411                    & <>\textbf{0.140}           & <>\textbf{0.653}           & <>246                     & <>9888                    & <>65.67                    & <>80.92                     & <>210                     & <>7787                    & <>\textbf{15.31}           & <>\textbf{10.03}           & <>503                     & <>16319                   & <>428.3                    & <>75.79                    \\
soc-digg                                       & <>770799                                   & <>5907132                                   & <>199                     & <>13551                   & <>\textbf{0.607}           & <>\textbf{69.97}           & <>5580                    & <>875610                  & <>NA                       & <>NA                        & <>519                     & <>37458                   & <>\textbf{29.27}           & <>\textbf{214.0}           & <>7349                    & <>1141673                 & <>NA                       & <>NA                       \\
socfb-Auburn71                                 & <>18448                                    & <>973918                                    & <>116                     & <>5780                    & <>\textbf{0.060}           & <>\textbf{8.102}           & <>1048                    & <>46693                   & <>23.01                    & <>27.51                     & <>323                     & <>14989                   & <>\textbf{5.589}           & <>\textbf{22.70}           & <>1624                    & <>73790                   & <>138.0                    & <>73.20                    \\
%socfb-Berkeley13                               & <>22900                                    & <>852419                                    & <>128                     & <>3776                    & <>\textbf{0.045}           & <>\textbf{3.776}           & <>925                     & <>29206                   & <>2.212                    & <>6.487                     & <>591                     & <>17281                   & <>\textbf{1.099}           & <>\textbf{15.50}           & <>10                      & <>1817                    & <>10.94                    & <>35.16                    \\
socfb-Cornell5                                 & <>18660                                    & <>790777                                    & <>211                     & <>6552                    & <>\textbf{0.056}           & <>\textbf{4.450}           & <>1292                    & <>52540                   & <>22.57                    & <>89.23                     & <>541                     & <>15848                   & <>\textbf{0.825}           & <>\textbf{22.60}           & <>2174                    & <>84381                   & <>44.67                    & <>107.1                    \\
socfb-Duke14                                   & <>9885                                     & <>506437                                    & <>198                     & <>4714                    & <>\textbf{0.054}           & <>\textbf{10.32}           & <>1489                    & <>56078                   & <>155.1                    & <>601.1                     & <>1042                    & <>34631                   & <>\textbf{39.14}           & <>\textbf{127.1}           & <>3375                    & <>134029                  & <>1416                     & <>1863                     \\
socfb-FSU53                                    & <>27737                                    & <>1034802                                   & <>188                     & <>8235                    & <>\textbf{0.052}           & <>\textbf{8.259}           & <>642                     & <>29659                   & <>39.75                    & <>34.89                     & <>401                     & <>18587                   & <>\textbf{1.161}           & <>\textbf{12.57}           & <>1025                    & <>45290                   & <>173.2                    & <>53.67                    \\
socfb-Indiana                                  & <>29732                                    & <>1305757                                   & <>136                     & <>4394                    & <>\textbf{0.036}           & <>\textbf{7.915}           & <>1596                    & <>57741                   & <>2.839                    & <>22.20                     & <>844                     & <>29290                   & <>\textbf{1.065}           & <>\textbf{17.54}           & <>2884                    & <>104681                  & <>16.84                    & <>151.5                    \\
socfb-Michigan23                               & <>30147                                    & <>1176516                                   & <>218                     & <>5764                    & <>\textbf{0.048}           & <>\textbf{5.805}           & <>1133                    & <>42875                   & <>2.090                    & <>13.34                     & <>542                     & <>18091                   & <>\textbf{0.658}           & <>\textbf{12.30}           & <>2378                    & <>95042                   & <>10.72                    & <>118.4                    \\
socfb-MIT                                      & <>6402                                     & <>251230                                    & <>203                     & <>4806                    & <>\textbf{0.044}           & <>\textbf{5.435}           & <>1099                    & <>35822                   & <>3.866                    & <>10.29                     & <>977                     & <>28110                   & <>\textbf{3.196}           & <>\textbf{35.87}           & <>1949                    & <>74120                   & <>36.62                    & <>76.38                    \\
socfb-Oklahoma97                               & <>17425                                    & <>892528                                    & <>79                      & <>2958                    & <>\textbf{0.049}           & <>\textbf{11.46}           & <>1148                    & <>61418                   & <>166.7                    & <>203.2                     & <>362                     & <>18706                   & <>\textbf{6.396}           & <>\textbf{16.35}           & <>1733                    & <>90058                   & <>615.2                    & <>234.1                    \\
socfb-OR                                       & <>63392                                    & <>816886                                    & <>152                     & <>2901                    & <>\textbf{0.075}           & <>\textbf{2.091}           & <>1440                    & <>35123                   & <>5.209                    & <>11.97                     & <>621                     & <>14999                   & <>\textbf{2.650}           & <>\textbf{23.49}           & <>4910                    & <>117554                  & <>42.24                    & <>510.8                    \\
socfb-Penn94                                   & <>41536                                    & <>1362220                                   & <>71                      & <>2228                    & <>\textbf{0.043}           & <>\textbf{4.693}           & <>875                     & <>23454                   & <>1.065                    & <>4.855                     & <>237                     & <>6564                    & <>\textbf{0.420}           & <>\textbf{7.032}           & <>2087                    & <>58201                   & <>2.863                    & <>34.31                    \\
socfb-Rice31                                   & <>4087                                     & <>184828                                    & <>83                      & <>1601                    & <>\textbf{0.033}           & <>\textbf{2.363}           & <>1170                    & <>36409                   & <>10.86                    & <>16.85                     & <>921                     & <>25731                   & <>\textbf{2.337}           & <>\textbf{35.17}           & <>2161                    & <>87191                   & <>80.34                    & <>141.8                    \\
socfb-Tennessee95                              & <>16979                                    & <>770659                                    & <>87                      & <>3604                    & <>\textbf{0.055}           & <>\textbf{4.836}           & <>802                     & <>31594                   & <>32.99                    & <>19.18                     & <>199                     & <>8737                    & <>\textbf{0.635}           & <>\textbf{10.03}           & <>1352                    & <>55156                   & <>72.43                    & <>36.94                    \\
socfb-Texas84                                  & <>36364                                    & <>1590651                                   & <>129                     & <>6606                    & <>\textbf{0.147}           & <>\textbf{8.989}           & <>927                     & <>41536                   & <>85.40                    & <>101.0                     & <>461                     & <>18985                   & <>\textbf{17.57}           & <>\textbf{40.66}           & <>1494                    & <>66131                   & <>600.9                    & <>398.6                    \\
socfb-UF                                       & <>35111                                    & <>1465654                                   & <>299                     & <>10983                   & <>\textbf{0.064}           & <>\textbf{15.21}           & <>1612                    & <>75851                   & <>54.72                    & <>82.69                     & <>975                     & <>42128                   & <>\textbf{5.514}           & <>\textbf{110.8}           & <>2088                    & <>98361                   & <>236.7                    & <>159.3                    \\
socfb-UGA50                                    & <>24389                                    & <>1174057                                   & <>125                     & <>6457                    & <>\textbf{0.099}           & <>\textbf{7.867}           & <>1276                    & <>55310                   & <>80.32                    & <>103.2                     & <>457                     & <>18956                   & <>\textbf{11.41}           & <>\textbf{39.75}           & <>2093                    & <>89760                   & <>471.5                    & <>286.4                    \\
socfb-Uillinois                                & <>30795                                    & <>1264421                                   & <>104                     & <>4828                    & <>\textbf{0.062}           & <>\textbf{6.582}           & <>586                     & <>25096                   & <>13.98                    & <>13.07                     & <>232                     & <>11219                   & <>\textbf{1.196}           & <>\textbf{8.368}           & <>1028                    & <>43222                   & <>76.21                    & <>27.78                    \\
socfb-UMass92                                  & <>16516                                    & <>519385                                    & <>142                     & <>3251                    & <>\textbf{0.034}           & <>1.636                    & <>634                     & <>14250                   & <>0.848                    & <>\textbf{1.489}            & <>523                     & <>12242                   & <>\textbf{0.819}           & <>\textbf{3.267}           & <>1440                    & <>37824                   & <>4.214                    & <>13.40                    \\
socfb-UVA16                                    & <>17196                                    & <>789321                                    & <>213                     & <>6905                    & <>\textbf{0.065}           & <>4.486                    & <>723                     & <>24976                   & <>2.724                    & <>\textbf{4.334}            & <>639                     & <>19899                   & <>\textbf{4.048}           & <>\textbf{22.61}           & <>1818                    & <>66673                   & <>38.56                    & <>55.52                    \\
socfb-Vassar85                                 & <>3068                                     & <>119161                                    & <>80                      & <>1220                    & <>\textbf{0.018}           & <>\textbf{0.654}           & <>940                     & <>22547                   & <>0.545                    & <>3.356                     & <>496                     & <>9340                    & <>\textbf{1.398}           & <>\textbf{18.27}           & <>2591                    & <>99363                   & <>7.661                    & <>220.9                    \\
socfb-Wisconsin87                              & <>23831                                    & <>835946                                    & <>122                     & <>3340                    & <>\textbf{0.037}           & <>\textbf{3.418}           & <>974                     & <>30242                   & <>4.655                    & <>8.164                     & <>727                     & <>20457                   & <>\textbf{2.280}           & <>\textbf{17.83}           & <>2371                    & <>72240                   & <>38.35                    & <>81.10                    \\
socfb-wosn-friends                             & <>63731                                    & <>817090                                    & <>152                     & <>2901                    & <>\textbf{0.075}           & <>\textbf{2.109}           & <>1440                    & <>35123                   & <>5.209                    & <>12.13                     & <>621                     & <>14999                   & <>\textbf{2.650}           & <>\textbf{24.45}           & <>4910                    & <>117554                  & <>42.24                    & <>514.0                    \\
socfb-Yale4                                    & <>8578                                     & <>405450                                    & <>140                     & <>3145                    & <>\textbf{0.026}           & <>\textbf{2.622}           & <>1033                    & <>28691                   & <>4.345                    & <>7.870                     & <>809                     & <>20248                   & <>\textbf{1.192}           & <>\textbf{31.41}           & <>2883                    & <>95160                   & <>31.38                    & <>160.6                    \\
Wiki-Vote                                      & <>7115                                     & <>100762                                    & <>85                      & <>1602                    & <>\textbf{0.104}           & <>\textbf{1.392}           & <>902                     & <>34228                   & <>182.2                    & <>430.5                     & <>1378                    & <>40535                   & <>\textbf{40.36}           & <>\textbf{170.8}           & <>2233                    & <>72679                   & <>NA                       & <>NA            \\ \bottomrule          
\end{tabular}
% }
\caption{Detailed results of KD-Club and KDBB on 32 representative MDCP instances from four benchmarks with $k = 3$ and $k=10$. The search tree size is in $10^4$, and the time is in seconds. The better results appear in bold.}
\label{tab-detailed-result}
\end{table*}
